Combating Human Trafficking with Deep Multimodal Models

Human trafficking is a global epidemic affecting millions of people across the planet. Sex trafficking, the dominant form of human trafficking, has seen a significant rise mostly due to the abundance of escort websites, where human traffickers can openly advertise among at-will escort advertisements. In this paper, we take a major step in the automatic detection of advertisements suspected to pertain to human trafficking. We present a novel dataset called Trafficking-10k, with more than 10,000 advertisements annotated for this task. The dataset contains two sources of information per advertisement: text and images. For the accurate detection of trafficking advertisements, we designed and trained a deep multimodal model called the Human Trafficking Deep Network (HTDN).

==> combating-human-trafficking-2 2/content/Abstract.tex <==
\par\noindent
\begin{abstract}
  Human trafficking is a global epidemic affecting millions of people across the planet.
  Sex trafficking, the dominant form of human trafficking, has seen a significant rise mostly due to the abundance of escort websites, where human traffickers can openly advertise among at-will escort advertisements.
  In this paper, we take a major step in the automatic detection of advertisements suspected to pertain to human trafficking.
  We present a novel dataset called Trafficking-10k, with more than 10,000~advertisements annotated for this task.
  The dataset contains two sources of information per advertisement: text and images.
  For the accurate detection of trafficking advertisements, we designed and trained a deep multimodal model called the Human Trafficking Deep Network (HTDN). 
\end{abstract}

==> combating-human-trafficking-2 2/content/Acknowledgements.tex <==
\section*{Acknowledgements}

We would like to thank William Chargin for creating figures and revising this paper.
We would also like to thank Torsten W\"ortwein for his assistance in visualizing our data.
Furthermore, we would like to thank our anonymous reviewers for their valuable feedback.
Finally, we would like to acknowledge collaborators from Marinus Analytics for the time and effort that they put into annotating advertisements for the dataset, and for allowing us to use their advertisement data.

==> combating-human-trafficking-2 2/content/Conclusion.tex <==
\section{Conclusion and Future Work}

In this paper, we took a major step in multimodal modeling of suspected online trafficking advertisements.
We presented a novel dataset, Trafficking-10k, with more than 10,000 advertisements annotated for this task.
The dataset contains two modalities of information per advertisement: text and images.
We designed a deep multimodal model called the Human Trafficking Deep Network (HTDN).
We compared the performance of the HTDN to various models that use language and vision alone.
The HTDN outperformed all of these, indicating that using information from both sources may be more helpful than using just one.

\textbf{Exploring language through character modeling.}
In order to eliminate the need for retraining the word vectors as the language of the domain evolves, we plan to use character models to learn a better language model for trafficking.
As new obfuscated words are introduced in escort advertisements, our hope is that character models will stay invariant to these obfuscations.
%One way to do so is learning the parameters of the language network with presence of manual obfuscation in the training data.
% ^ What does this mean? :(

\textbf{Understanding images.}
While CNNs have proven to be useful for many different computer vision tasks, we seek to improve the learning capability of the visual network.
Future direction involves using graphical modeling to understand interactions in the scene.
Another direction involves working to understand text in images, which can provide more information about the subjects of the images.

Given that the current state of the art in this area generally does not use deep models, this may be a major opportunity for improvement.
To this end, we encourage the research community to reach out to Cara Jones, an author of this paper, to obtain a copy of Trafficking-10k and other training data.

==> combating-human-trafficking-2 2/content/Dataset.tex <==
\section{Trafficking-10k Dataset}

In this section, we present the dataset for our studies.
We formalize the problem of recognizing sex trafficking as a machine learning task.
The input data is text and images; this is mapped to a measure of how suspicious the advertisement is with regards to human trafficking.%
\input{figs/USMapFig} %
\subsection{Data Acquisition and Preprocessing}
A subset of 10,000 ads were sampled randomly from a large cache of escort ads for annotation in Trafficking-10k dataset.
The distribution of advertisements across the United States and Canada is shown in Figure~\ref{fig:usmap}, which indicates the diversity of advertisements in Trafficking-10k. This diversity ensures that models trained on Trafficking-10k can be applicable nationwide.
%Furthermore, it enables studies that target differences in dynamics of trafficking depending on geographic location.
% Above sentence struck because T10k does not include geographic data.
The 10,000 collected ads each consist of text and zero or more images.
The text in the dataset is in plain text format, derived by stripping the HTML tags from the raw source of the ads.
%The text was derived from the raw HTML of advertisements;
%As the first step in preprocessing text, the HTML tags are stripped and only the content of the ads are considered important.
The set of characters in each advertisement is encoded as UTF-8, because there is ample usage of smilies and non-English characters.
%Unlike HTML tags, these characters are informative since they are semantically meaningful, such as dollar sign smiley representing only-cash exchange.
Advertisements are truncated to the first 184~words, as this covers more than 90\% of the ads. Images are resized to $224 \times 224$ pixels with RGB channels.

\subsection{Trafficking Annotation}
Detecting whether or not an advertisement is suspicious requires years of practice and experience in working closely with law enforcement.
As a result, annotation is a highly complicated and expensive process, which cannot be scaled using crowdsourcing.
In our dataset, annotation is carried out by two expert annotators, each with at least five years of experience, in detection of human trafficking and another annotator with one year of experience.
In our dataset, annotations were done by three experts.
One expert has over a year of experience, and the other two have over five years of experience in the human trafficking domain.
%To calculate the inter-annotator agreement, each annotator is given a set of 1,000 similar ads to annotate.
% TODO: This is wrong. Edmund to fix
To calculate the inter-annotator agreement, each annotator is given the same set of 1000 ads to annotate and the nominal agreement is found: there was a 83\% pairwise agreement (0.62 Krippendorff's alpha).
Also, to make sure that annotations are generalizable across the annotators and law enforcement officers, two law enforcement officers annotated, respectively, a subset of 500 and 100 of the advertisements. 
We found a 62\% average pairwise agreement (0.42 Krippendorff's alpha) with our annotators.
This gap is reasonable, as law enforcement officers only have experience with local advertisements, while Trafficking-10k annotators have experience with cases across the United States. %

Annotators used an annotation interface specifically designed for the Trafficking-10k dataset.
In the annotation interface, each advertisement was displayed on a separate webpage.
The order of the advertisements is determined uniformly randomly, and annotators were unable to move to the next advertisement without labeling the current one.
For each advertisement, the annotator was presented with the question: ``In your opinion, would you consider this advertisement suspicious of human trafficking?''
The annotator is presented with the following options: ``Certainly no,'' ``Likely no,'' ``Weakly no,'' ``Unsure,''\footnote{This option is greyed out for 10~seconds to encourage annotators to make an intuitive decision.} ``Weakly yes,'' ``Likely yes,'' and ``Certainly yes.''
Thus, the degree to which advertisements are suspicious is quantized into seven levels.

\subsection{Analysis of Language}

The language used in these advertisements introduces fundamental challenges to the field of NLP.
The nature of the textual content in these advertisements raises the question of how we can make inferences in a linguistic environment with a constantly evolving lexicon.
Language used in the Trafficking-10k dataset is highly inconsistent with standard grammar.
Often, words are obfuscated by emojis and symbols.
The word ordering is inconsistent, and there is rarely any form of constituency.
This form of language is completely different from spoken and written English.
These attributes make escort advertisements appear somewhat similar to tweets, specifically since these ads are normally short (more than~90\% of the ads have at most 184~words).
Another point of complexity in these advertisements is the high number of unigrams, due to usage of uncommon words and obfuscation.
On top of unigram complexity, advertisers continuously change their writing pattern, making this problem more complex.

\input{figs/AdLength}
\subsection{Dataset Statistics}

There are 106,954 distinct unigrams, 353,324 distinct bigrams, and 565,403 trigrams in the Trafficking-10k dataset.
There are 60,337 images.
The total number of distinct characters including whitespace, punctuations, and hex characters is~182.
The average length of an ad is~137 words, with a standard deviation of~74, median~133.
The shortest advertisement has 7~unigrams, and the longest advertisement has 1810~unigrams.
There are of 106,954 distinct unigrams, 353,324 distinct bigrams and 565,403 trigrams in the Trafficking-10k dataset.
The average number of images in an advertisement is~5.9; the median is~5, the minimum is~0, and the maximum is~90.

The length of \emph{suspected} advertisements is 134 unigrams; the standard deviation is 39, the minimum is 12, and the maximum is 666.
The length of \emph{non-suspected} ads is 141; the standard deviation is 85, the minimum is 7, and the maximum is 1810.
The total number of suspected ads is~3257; and the total number of non-suspected ads is~6992.
Figure~\ref{fig:adlen} shows the histogram of number of ads based on their length. Both the positive and negative distributions are similar. This means that there is no obvious length difference between the two classes.
Most of the ads have a length of~80--180 words.


==> combating-human-trafficking-2 2/content/Experiments.tex <==
\section{Experiments}

In our experiments, we compare the HTDN with previously used approaches for detection of trafficking suspicious ads.
Furthermore, we compare the HTDN to the performance of its unimodal components.
In all our experiments we perform binary classification of whether the advertisement is suspected of being related to trafficking.
The main comparison method that we use is the weighted accuracy and F1-score (due to imbalance it dataset).
The formulation for weighted accuracy is as follows:
\begin{equation}
  \mathrm{Wt.\ Acc.} = \frac{\mathrm{TP} \times \mathrm{N} / \mathrm{P} + \mathrm{TN}}{2 \mathrm{N}}
\end{equation}
where $\mathrm{TP}$ (resp.\ $\mathrm{TN}$) is true positive (resp.\ true negative) predictions, and $\mathrm{P}$ (resp.\ $\mathrm{N}$) is the total number of positive (resp.\ negative) examples.


\subsection{Baselines}

We compare the performance of the HTDN network with baseline models divided in 4 major categories

\textbf{Bag-of-Words Baselines.}
This set of baselines is designed to assess performance of off-the-shelf basic classifiers and basic language features.
We train random forest, logistic regression and linear SVMs to show the performance of simple language-only models.

\textbf{Keyword Baselines.}
These demonstrate the performance of models that use a set of 108 keywords, all highly related to trafficking, provided by law enforcement officers.%
\footnote{%
  Not presented in this paper due to sensitive nature of these keywords.
}
A binary one-hot vector representing these keywords is used to train the random forest, logistic regression, and linear SVM models.

\textbf{108 One-Hot Baselines.}
Similar to Keywords Baseline, we use feature selection technique to filter the most informative 108 words for detection of trafficking. We compare the performance of this baseline to Keywords baseline to evaluate the usefulness of expert knowledge in keywords selection vs automatic data-driven keyword selection.

\textbf{Average Trafficking Vectors Baselines.}
We assess the magnitude of success for the trafficking word embeddings for different classifiers.
For the random forest, logistic regression, and linear SVM models, the average word vector is calculated and used as input.

\textbf{HTDN Unimodal.}
These baselines show the performance of unimodal components of HTDN. For language we only use $\mathcal{F}_l$ component of the pipeline and for visual we use $\mathcal{F}_v$, using both pre-trained a VGG and finetuned T-VGG.

\textbf{Random and Human.}
Random is based on assigning the more frequent class in training set to all the test data, and can be considered a lower bound for our model. Human performance metrics are upper bounds for this task's metrics.

We visualize the different inputs to our baseline models to show the complexity of the dataset when using different feature sets.
Figure~\ref{fig:tsne} shows the 2D t-SNE \cite{maaten2008visualizing} representation of the training data in our dataset according to the Bag-of-Words (top right) models, expert keywords (top left), average word vectors (bottom right), and the visual representation $h_v$ bottom left.
The distribution of points suggests that none of the feature representations make the classification task trivial.

\subsection{Training Parameters}

All the models in our experiments are trained on the Trafficking-10k designated training set and tested on the designated test set.
Hyperparameter evaluation is performed using a subset of training set as validation set.
The HTDN model is trained using the Adam optimizer \cite{kingma2014adam}.
The neural weights were initialized randomly using Xavier initialization technique \cite{glorot2010understanding}.
The random forest model uses $10$~estimators, with no maximum depth, and minimum-samples-per-split value of 2.
The linear SVM model uses an $\ell_2$-penalty and a square hinge loss with $C = 1$.

==> combating-human-trafficking-2 2/content/Introduction.tex <==
\section{Introduction}
Human trafficking ``a crime that shames us all'' \cite{unodc2008}, has seen a steep rise in the United States since~2012.
The number of cases reported rose from 3,279 in~2012 to 7,572 in~2016---more than doubling over the course of five years \cite{hotline2017}. 
%Sex trafficking is the most common form of human trafficking and is a global epidemic affecting millions of men, women, and children each year \cite{mccarthy2014human}.
% The above source does not seem to support the claim. Indeed, it states the following:
% ``A focus on sex trafficking means that these other forms of exploitation often go unrecognized and other areas of policy that could lower the risks of exploitation tend to be ignored.''
Sex trafficking is a form of human trafficking, and is a global epidemic affecting millions of people each year \cite{mccarthy2014human}.
%The UN estimates that it is the world's fastest growing type of organized crime and the third most common in the world.%
%\footnote{\url{http://goo.gl/UaX0G7}}
% Removed: Source does not support claim.
Victims of sex trafficking are subjected to coercion, force, and control, and are not able to ask for help.
Put plainly, sex trafficking is modern-day slavery and is one of the top priorities of law enforcement agencies at all levels.

A major advertising ground for human traffickers is the World Wide Web.
The Internet has brought traffickers the ability to advertise online and has fostered the growth of numerous adult escort sites.
Each day, there are tens of thousands of Internet advertisements posted in the United States and Canada that market commercial sex.
Hiding among the noise of at-will adult escort ads are ads posted by sex traffickers.
Often long undetected, trafficking rings and escort websites form a profit cycle that fuels the increase of both trafficking rings and escort websites.
% Above claim unsubstantiated.

For law enforcement, this presents a significant challenge: how should we identify advertisements that are associated with sex trafficking?
Police have limited human and technical resources, and manually sifting through thousands of ads in the hopes of finding something suspicious is a poor use of those resources, even if they know what they are looking for.
Leveraging state-of-the-art machine learning approaches in~Natural Language Processing and computer vision to detect and report advertisements suspected of trafficking is the main focus of our work.
In other words, we strive to find the victims and perpetrators of trafficking who hide in plain sight in the massive amounts of data online.
By narrowing down the number of advertisements that law enforcement must sift through, we endeavor to provide a real opportunity for law enforcement to intervene in the lives of victims.
However, there are non-trivial challenges facing this line of research:

\textbf{Adversarial Environment.}
Human trafficking rings are aware that law enforcement monitors their online activity.
Over the years, law enforcement officers have populated lists of keywords that frequently occur in trafficking advertisements.
However, these simplistic queries fail when traffickers use complex obfuscation.
Traffickers, again aware of this, move to new keywords to blend in with the at-will escort advertisements.
This trend creates an adversarial environment for any machine learning system that attempts to find trafficking rings hiding in plain sight.

\textbf{Defective Language Compositionality.}
Online escort advertisements are difficult to analyze, because they lack grammatical structures such as constituency.
Therefore, any form of inference must rely more on context than on grammar.
This presents a significant challenge to the NLP community.
Furthermore, the majority of the ads contain emojis and non-English characters.

\textbf{Generalizable Language Context.}
Machine learning techniques can easily learn unreliable cues in training sets such as phone numbers, keywords, and other forms of semantically unreliable discriminators to reduce the training loss.
Due to limited similarity between the training and test data due to the large number of ads available online, relying on these cues is futile.
Learned discriminative features should be generalizable and model semantics of trafficking.

\textbf{Multimodal Nature.}
Escort advertisements are composed of both textual and visual information.
Our model should treat these features interdependently. 
For instance, if the text indicates that the escort is in a hotel room, our model should consider the effect that such knowledge may have on the importance of certain visual features.
% TODO: Consider \emph{}asizing both ``text'' and ``visual.''

We believe that studying human trafficking advertisements can be seen as a fundamental challenge to the NLP, computer vision, and machine learning communities dealing with language and vision problems.
In this paper, we present the following contributions to this research direction.
First, we study the language and vision modalities of the escort advertisements through deep neural modeling.
%While there are similarities in the text and images used in these advertisements with text and images used in tweets and reviews, there are fundamental differences that are distinguishable to research in this area.
Second, we take a significant step in automatic detection of advertisements suspected of sex trafficking.
While previous methods \cite{dubrawski2015leveraging} have used simplistic classifiers, we build an end-to-end-trained multimodal deep model called the Human Trafficking Deep Network (HTDN).
The HTDN uses information from both text and images to extract cues of human trafficking, and shows outstanding performance compared to previously used models.
Third, we present the first rigorously annotated dataset for detection of human trafficking, called Trafficking-10k, which includes more than 10,000 trafficking ads labeled with likelihoods of having been posted by traffickers.%
\footnote{%
  Due to the sensitive nature of this dataset, access can only be granted by emailing Cara Jones.
  Different levels of access are provided \emph{only} to scientific community.
}
%https://humantraffickinghotline.org/sites/default/files/NHTRC%202015%20United%20States%20Report%20-%20USA%20-%2001.01.15%20-%2012.31.15_OTIP_Edited_06-09-16.pdf

==> combating-human-trafficking-2 2/content/Model.tex <==
\section{Model}

In this section, we present our deep multimodal network called the Human Trafficking Deep Network (HTDN).
The HTDN is a multimodal network with language and vision components.
The input to the HTDN is an ad, text and images.
The HTDN is shown in Figure~\ref{fig:overview}.
In the remainder of this section, we will outline the different parts of the HTDN, and the input features to each component.

\subsection{Trafficking Word Embeddings}

Our approach to deal with the adversarial environment of escort ads is to use word vectors, defining words not based on their constituent characters, but rather based on their context.
For instance, consider the two unigrams ``cash'' and ``\copyright a\$h.''
While these contain different characters, semantically they are the same, and they occur in the same context.
Thus, our expectation is that both the unigrams will be mapped to similar vectors.
Word embeddings pre-trained on general domains do not cover most of the unigrams in Trafficking-10k.
For instance, the GloVe embedding \cite{pennington2014glove} trained on Wikipedia covers only~49.7\% of our unigrams.
The first step of the HTDN pipeline is to train word vectors \cite{mikolov2013distributed} based on the skip-gram model.
This is especially suitable for escort ads, because skip-gram models are able to capture context without relying on word order.
We train the word embedding using 1,000,000 unlabeled ads from a dataset that does not include the Trafficking-10k data.
For each advertisement, the input to the trained embedding is a sequence of words $\mathbf{\hat{w}} = [\hat{w}_1, \dotsc, \hat{w}_t]$, and the output is a sequence of $100$-dimensional word vectors $\mathbf{w} = [w_1, \dotsc, w_t]$, where $t$ is the size of the advertisement and $w_i \in \mathbb{R}^{100}$.
Our trained word vectors cover 94.9\% of the unigrams in the Trafficking-10k dataset.

\subsection{Language Network}

Our language network is designed to deal with two challenging aspects of escort advertisements: (1)~violation of constituency, and (2)~presence of irrelevant information not related to trafficking but present in ads. We address both of these issues by learning a time dependent embedding at word level. This allows the model to not rely on constituency and also remember useful information from the past, should the model get overwhelmed by irrelevant information. 
Our proposed language network, $\mathcal{F}_l$, takes as input a sequence of word vectors $\mathbf{w} = [w_1, \dotsc, w_t]$, and outputs a neural language representation $h_l$.
As a first step, $\mathcal{F}_l$ uses the word embeddings as input to a Long-Short Term Memory (LSTM) network and produces a new supervised context-aware word embedding $\mathbf{u} = [u_1, \dotsc, u_t]$ where $u_i \in \mathbb{R}^{300}$ is the output of the LSTM at time $i$.
Then, $\mathbf{u}$ is fed into a fully connected layer with dropout $p = 0.5$ to produce the neural language representation $h_l \in \mathbb{R}^{300}$ according to the following formulas with weights $W_l$ for the LSTM and implicit weights in the fully connected layers, which we represent by $\mathit{FC}$:
\begin{align}
  u_i &= \mathit{LSTM}(i, w_i; W_l) \\
  \mathbf{u} &= [u_1, \dotsc, u_t] \\
  h_l &= \mathit{FC}(\mathbf{u}).
\end{align}
The generated $h_l$ is then used as part of the HTDN pipeline, and is also trained independently to assess the performance of the language-only model.
The language network $\mathcal{F}_l$ is the combination of the LSTM and the fully-connected network.

\subsection{Vision Network}

Parallel to the language network, the vision network $\mathcal{F}_v$ takes as input advertisement images and extracts visual representations $h_v$.
The vision network takes at most five images; the median number of images per advertisement in Trafficking-10k is~$5$.
To learn contextual and abstract information from images, we use a deep convolutional neural network called Trafficking-VGG (T-VGG), a fine-tuned instance of the well-known VGG~network \cite{simonyan2014very}.
T-VGG is a deep model with $13$ consecutive convolutional layers followed by $2$ fully connected layers; it does not include the softmax layer of~VGG.
The procedure for fine-tuning T-VGG maps each individual image to a label that comes from the advertisement, and then performs end-to-end training.
For example, if there are five images in an advertisement with positive label, all five images are mapped to positive label.
After fine-tuning, three fully connected layers of 200~neurons with dropout $p = 0.5$ are added to the network.
The combination of T-VGG and the fully connected layers is the vision network $\mathcal{F}_l$.
We consider five images $\boldsymbol{\hat{\imath}} = \{ \hat{\imath}_1, \dotsc, \hat{\imath}_5 \}$ from each input advertisement.
If the advertisement has fewer than five images, zero-filled images are added.
For each image, the output of $\mathcal{F}_v$ is a representation of five images $\mathbf{i} = \{ i_1, \dotsc, i_5 \}$.
The visual representation $h_v \in \mathbb{R}^{5 \times 200}$ is a matrix with a size-$200$ representation of each of the $5$~images:
\begin{align}
  h_v = \mathcal{F}_v(\boldsymbol{\hat{\imath}}; W_v).
\end{align}

\subsection{Multimodal Fusion}

Escort advertisements have complex dynamics between text and images.
Often, neither linguistic nor visual cues alone can suffice to classify whether an ad is suspicious. Interactions between linguistic and visual cues can be non-trivial, so this requires an explicit joint representation for each neuron in the linguistic and visual representations. 
In our multimodal fusion approach we address this by calculating an outer product between language and visual representations $h_l$ and $h_v$ to build the full space of possible outcomes: 
\begin{equation}
  h_m = h_l \otimes h_v,
\end{equation}
where $\otimes$ is an outer product of the two representations.
This creates a joint multimodal tensor called $h_m$ for language and visual modalities.
In this tensor, every neuron in the language representation is multiplied by every neuron in vision representation, thus creating a new representation containing the information of both of them.
Thus, the final fusion tensor $h_m \in \mathbb{R}^{5 \times 200 \times 300}$ contains information from the joint interaction of the language and visual modalities.

\subsection{Convolutional Decision Network}

The multimodal representation $h_m$ is used as the input to the convolutional decision network $\mathcal{F}_d$.
%The first dimension in $h_m$ is considered the depth, and the other two dimensions are width and height.
$\mathcal{F}_d$ has two layers of convolution and max pooling with a dropout rate of $p = 0.5$, followed by a fully connected layer of $150$~neurons with a dropout rate of $p = 0.5$.
Performing convolutions in this space enables the model to attend to small areas of linguistic and visual cues.
It can thus find correspondences between specific combinations of the linguistic and visual representations.
The final decision is made by a single sigmoid neuron.
%with probability given by
%\begin{equation}
%  \label{eq:SIN}
%  \argmax_{\tau} \ \Pr(\tau \mid \mathbf{h}_m; W_d) = \argmax_{\tau} \ \mathcal{F}_d(\mathbf{h}_m ; W_d),
%\end{equation}
%where $\tau \in \{ 0, 1 \}$ indicates whether an advertisement is perceived as suspicious, and $W_d$ is the set of learnable weights for $\mathcal{F}_d$.

==> combating-human-trafficking-2 2/content/RelatedWorks.tex <==
\section{Related Works}

Automatic detection of human trafficking has been a relatively unexplored area of machine learning research.
Very few machine learning approaches have been proposed to detect signs of human trafficking online.
Most of these approaches use simplistic methods such as multimedia matching \cite{zhou2016multimedia}, text-based filtering classifiers such as random forests, logistic regression, and SVMs \cite{dubrawski2015leveraging}, and named-entity recognition to isolate the instances of trafficking \cite{nagpal2015entity}.
Studies have suggested using statistical methods to find keywords and signs of trafficking from data to help law enforcement agencies \cite{kennedy2012predictive} as well as adult content filtering using textual information \cite{zhou2016multimedia}.

Multimodal approaches have gained popularity over the past few years.
These multimodal models have been used for medical purposes, such as detection of suicidal risk, PTSD and depression \cite{scherer2016self,venek2016adolescent,yu2013multimodal,valstar2016avec}; sentiment analysis \cite{zadeh2016multimodal,poria2016convolutional,zadeh2016mosi}; emotion recognition \cite{poria2017review}; image captioning and media description \cite{you2016image, donahue2015long}; question answering \cite{antol2015vqa}; and multimodal translation \cite{specia2016shared}.

To the best of our knowledge, this paper presents the first multimodal and deep model for detection of human trafficking. 

==> combating-human-trafficking-2 2/content/ResultsDiscussion.tex <==
\section{Results and Discussion}

The results of our experiments are shown in Table~\ref{table:results}.
We report the results on three metrics: F1-score, weighted accuracy, and accuracy.
Due to the imbalance between the numbers of positive and negative samples, weighted accuracy is more informative than unweighted accuracy, so we focus on the former.

\textbf{HTDN.}
The first observation from Table~\ref{table:results} is that the HTDN model outperforms all the proposed baselines.
There is a significant gap between the HTDN (and variants) and other non-neural approaches.
This better performance is an indicator of complex interactions in detecting dynamics of human trafficking, which is captured by the HTDN.

\textbf{Both Modalities are Helpful.}
Both modalities are helpful in predicting signs of trafficking ($\mathcal{F}_l$ and $\mathcal{F}_v$ [T-VGG]).
Fine-tuning VGG network parameters shows improvement over pre-trained VGG parameters.

\textbf{Language is More Important.}
Since $\mathcal{F}_l$ shows better performance than $\mathcal{F}_v$ [T-VGG], the language modality appears to be the more informative modality for detecting trafficking suspicious ads. 

%% This section is unsubstantiated.
%\textbf{Law Enforcement Keywords.}
%Our results indicate that reducing the feature set to set of keywords provided by the law-enforcement hurts the performance of the model.
%This indicates that keyword searching commonly used by law enforcement agencies may hurt the performance of the search queries or automatic systems currently being used by agencies.
%Also, because obfuscation is widely used in escort advertisement websites, these keywords may not generalize.
%The same is true for feature set reduction using feature selection. 

==> combating-human-trafficking-2 2/content/done.tex <==
-- Statistics for the ads, how many unigrams (106954), images (60337), bigrams (353324), trigrams (565403), characters including spaces and punctuation and hex, excluding newline (182), average length of ad (avg 137 words, stddev 74, median 133, min 7, max 1810), average number of images (avg 5.9, median 5, mode 4, stddev 4.6, min 0, max 90), average length of trafficking ads (avg 134 words, stddev 39, median 136, min 12, max 666) , average length of non-trafficking ads (avg 141, stddev 85, median 131, min 7, max 1810), number of trafficking ads (3257), number of non-trafficking ads (6992), couple of other ideas for visualizing the trafficking stuff, such as look at MOSI sentiment paper figure 2. 9

-- How many n-grams are out if we use glove 9
-- Recalculate f1. 
-- Overview figure -- william

==> combating-human-trafficking-2 2/content/dummy.tex <==
\iffalse
\begin{figure*}
\centering
\begin{tikzpicture}
\begin{axis}[
xlabel style={font={\small}},
xlabel={Hey!},
legend pos={outer north east},
width=5in,
title=Hello,
]
\addplot table {fscorevsubprob.dat};
\addlegendentry{RF-F}
\addplot table[y index={2}] {fscorevsubprob.dat};
\addlegendentry{SVM-F}
\addplot table[y index={3}] {fscorevsubprob.dat};
\addlegendentry{LR-F}
\addplot table[y index={4}] {fscorevsubprob.dat};
\addlegendentry{cLSTM-F}
\end{axis}
\end{tikzpicture}
\end{figure*}
\fi
\iffalse
\section{Credits}

This document has been adapted from the instructions for earlier ACL
and NAACL proceedings, including those for ACL 2017 by Dan Gildea and
Min-Yen Kan, NAACL-2017 by Margaret Mitchell, ACL-2012 by Maggie Li
and Michael White, those from ACL-2010 by Jing-Shing Chang and Philipp
Koehn, those for ACL-2008 by Johanna D. Moore, Simone Teufel, James
Allan, and Sadaoki Furui, those for ACL-2005 by Hwee Tou Ng and Kemal
Oflazer, those for ACL-2002 by Eugene Charniak and Dekang Lin, and
earlier ACL and EACL formats. Those versions were written by several
people, including John Chen, Henry S. Thompson and Donald
Walker. Additional elements were taken from the formatting
instructions of the {\em International Joint Conference on Artificial
  Intelligence} and the \emph{Conference on Computer Vision and
  Pattern Recognition}.

\section{Introduction}

The following instructions are directed to authors of papers submitted
to ACL-2017 or accepted for publication in its proceedings. All
authors are required to adhere to these specifications. Authors are
required to provide a Portable Document Format (PDF) version of their
papers. \textbf{The proceedings are designed for printing on A4
paper.}

\section{General Instructions}

Manuscripts must be in two-column format.  Exceptions to the
two-column format include the title, authors' names and complete
addresses, which must be centered at the top of the first page, and
any full-width figures or tables (see the guidelines in
Subsection~\ref{ssec:first}). {\bf Type single-spaced.}  Start all
pages directly under the top margin. See the guidelines later
regarding formatting the first page.  The manuscript should be
printed single-sided and its length
should not exceed the maximum page limit described in Section~\ref{sec:length}.
Pages are numbered for  initial submission. However, {\bf do not number the pages in the camera-ready version}.

By uncommenting {\small\verb|\aclfinalcopy|} at the top of this 
 document, it will compile to produce an example of the camera-ready formatting; by leaving it commented out, the document will be anonymized for initial submission.  When you first create your submission on softconf, please fill in your submitted paper ID where {\small\verb|***|} appears in the {\small\verb|\def\aclpaperid{***}|} definition at the top.

The review process is double-blind, so do not include any author information (names, addresses) when submitting a paper for review.  
However, you should maintain space for names and addresses so that they will fit in the final (accepted) version.  The ACL 2017 \LaTeX\ style will create a titlebox space of 2.5in for you when {\small\verb|\aclfinalcopy|} is commented out.  

\subsection{The Ruler}
The ACL 2017 style defines a printed ruler which should be presented in the
version submitted for review.  The ruler is provided in order that
reviewers may comment on particular lines in the paper without
circumlocution.  If you are preparing a document without the provided
style files, please arrange for an equivalent ruler to
appear on the final output pages.  The presence or absence of the ruler
should not change the appearance of any other content on the page.  The
camera ready copy should not contain a ruler. (\LaTeX\ users may uncomment
the {\small\verb|\aclfinalcopy|} command in the document preamble.)  

Reviewers: note that the ruler measurements do not align well with
lines in the paper -- this turns out to be very difficult to do well
when the paper contains many figures and equations, and, when done,
looks ugly. In most cases one would expect that the approximate
location will be adequate, although you can also use fractional
references ({\em e.g.}, the first paragraph on this page ends at mark $114.5$).

\subsection{Electronically-available resources}

ACL provides this description in \LaTeX2e{} ({\small\tt acl2017.tex}) and PDF
format ({\small\tt acl2017.pdf}), along with the \LaTeX2e{} style file used to
format it ({\small\tt acl2017.sty}) and an ACL bibliography style ({\small\tt acl\_natbib.bst})
and example bibliography ({\small\tt acl2017.bib}).
These files are all available at
{\small\tt acl2017.org/index.php?article\_id=9}. We
strongly recommend the use of these style files, which have been
appropriately tailored for the ACL 2017 proceedings.

\subsection{Format of Electronic Manuscript}
\label{sect:pdf}

For the production of the electronic manuscript you must use Adobe's
Portable Document Format (PDF). PDF files are usually produced from
\LaTeX\ using the \textit{pdflatex} command. If your version of
\LaTeX\ produces Postscript files, you can convert these into PDF
using \textit{ps2pdf} or \textit{dvipdf}. On Windows, you can also use
Adobe Distiller to generate PDF.

Please make sure that your PDF file includes all the necessary fonts
(especially tree diagrams, symbols, and fonts with Asian
characters). When you print or create the PDF file, there is usually
an option in your printer setup to include none, all or just
non-standard fonts.  Please make sure that you select the option of
including ALL the fonts. \textbf{Before sending it, test your PDF by
  printing it from a computer different from the one where it was
  created.} Moreover, some word processors may generate very large PDF
files, where each page is rendered as an image. Such images may
reproduce poorly. In this case, try alternative ways to obtain the
PDF. One way on some systems is to install a driver for a postscript
printer, send your document to the printer specifying ``Output to a
file'', then convert the file to PDF.

It is of utmost importance to specify the \textbf{A4 format} (21 cm
x 29.7 cm) when formatting the paper. When working with
{\tt dvips}, for instance, one should specify {\tt -t a4}.
Or using the command \verb|\special{papersize=210mm,297mm}| in the latex
preamble (directly below the \verb|\usepackage| commands). Then using 
{\tt dvipdf} and/or {\tt pdflatex} which would make it easier for some.

Print-outs of the PDF file on A4 paper should be identical to the
hardcopy version. If you cannot meet the above requirements about the
production of your electronic submission, please contact the
publication chairs as soon as possible.

\subsection{Layout}
\label{ssec:layout}

Format manuscripts two columns to a page, in the manner these
instructions are formatted. The exact dimensions for a page on A4
paper are:

\begin{itemize}
\item Left and right margins: 2.5 cm
\item Top margin: 2.5 cm
\item Bottom margin: 2.5 cm
\item Column width: 7.7 cm
\item Column height: 24.7 cm
\item Gap between columns: 0.6 cm
\end{itemize}

\noindent Papers should not be submitted on any other paper size.
 If you cannot meet the above requirements about the production of 
 your electronic submission, please contact the publication chairs 
 above as soon as possible.

\subsection{Fonts}

For reasons of uniformity, Adobe's {\bf Times Roman} font should be
used. In \LaTeX2e{} this is accomplished by putting

\begin{quote}
\begin{verbatim}
\usepackage{times}
\usepackage{latexsym}
\end{verbatim}
\end{quote}
in the preamble. If Times Roman is unavailable, use {\bf Computer
  Modern Roman} (\LaTeX2e{}'s default).  Note that the latter is about
  10\% less dense than Adobe's Times Roman font.

\begin{table}[h]
\begin{center}
\begin{tabular}{|l|rl|}
\hline \bf Type of Text & \bf Font Size & \bf Style \\ \hline
paper title & 15 pt & bold \\
author names & 12 pt & bold \\
author affiliation & 12 pt & \\
the word ``Abstract'' & 12 pt & bold \\
section titles & 12 pt & bold \\
document text & 11 pt  &\\
captions & 11 pt & \\
abstract text & 10 pt & \\
bibliography & 10 pt & \\
footnotes & 9 pt & \\
\hline
\end{tabular}
\end{center}
\caption{\label{font-table} Font guide. }
\end{table}

\subsection{The First Page}
\label{ssec:first}

Center the title, author's name(s) and affiliation(s) across both
columns. Do not use footnotes for affiliations. Do not include the
paper ID number assigned during the submission process. Use the
two-column format only when you begin the abstract.

{\bf Title}: Place the title centered at the top of the first page, in
a 15-point bold font. (For a complete guide to font sizes and styles,
see Table~\ref{font-table}) Long titles should be typed on two lines
without a blank line intervening. Approximately, put the title at 2.5
cm from the top of the page, followed by a blank line, then the
author's names(s), and the affiliation on the following line. Do not
use only initials for given names (middle initials are allowed). Do
not format surnames in all capitals ({\em e.g.}, use ``Mitchell'' not
``MITCHELL'').  Do not format title and section headings in all
capitals as well except for proper names (such as ``BLEU'') that are
conventionally in all capitals.  The affiliation should contain the
author's complete address, and if possible, an electronic mail
address. Start the body of the first page 7.5 cm from the top of the
page.

The title, author names and addresses should be completely identical
to those entered to the electronical paper submission website in order
to maintain the consistency of author information among all
publications of the conference. If they are different, the publication
chairs may resolve the difference without consulting with you; so it
is in your own interest to double-check that the information is
consistent.

{\bf Abstract}: Type the abstract at the beginning of the first
column. The width of the abstract text should be smaller than the
width of the columns for the text in the body of the paper by about
0.6 cm on each side. Center the word {\bf Abstract} in a 12 point bold
font above the body of the abstract. The abstract should be a concise
summary of the general thesis and conclusions of the paper. It should
be no longer than 200 words. The abstract text should be in 10 point font.

{\bf Text}: Begin typing the main body of the text immediately after
the abstract, observing the two-column format as shown in 
the present document. Do not include page numbers.

{\bf Indent}: When starting a new paragraph. Use 11 points for text and 
subsection headings, 12 points for section headings and 15 points for
the title. 

\begin{table}
\centering
\small
\begin{tabular}{cc}
\begin{tabular}{|l|l|}
\hline
{\bf Command} & {\bf Output}\\\hline
\verb|{\"a}| & {\"a} \\
\verb|{\^e}| & {\^e} \\
\verb|{\`i}| & {\`i} \\ 
\verb|{\.I}| & {\.I} \\ 
\verb|{\o}| & {\o} \\
\verb|{\'u}| & {\'u}  \\ 
\verb|{\aa}| & {\aa}  \\\hline
\end{tabular} & 
\begin{tabular}{|l|l|}
\hline
{\bf Command} & {\bf  Output}\\\hline
\verb|{\c c}| & {\c c} \\ 
\verb|{\u g}| & {\u g} \\ 
\verb|{\l}| & {\l} \\ 
\verb|{\~n}| & {\~n} \\ 
\verb|{\H o}| & {\H o} \\ 
\verb|{\v r}| & {\v r} \\ 
\verb|{\ss}| & {\ss} \\\hline
\end{tabular}
\end{tabular}
\caption{Example commands for accented characters, to be used in, {\em e.g.}, \BibTeX\ names.}\label{tab:accents}
\end{table}

\subsection{Sections}

{\bf Headings}: Type and label section and subsection headings in the
style shown on the present document.  Use numbered sections (Arabic
numerals) in order to facilitate cross references. Number subsections
with the section number and the subsection number separated by a dot,
in Arabic numerals. Do not number subsubsections.

\begin{table*}
\centering
\begin{tabular}{lll}
  output & natbib & previous ACL style files\\
  \hline
  \citep{Gusfield:97} & \verb|\citep| & \verb|\cite| \\
  \citet{Gusfield:97} & \verb|\citet| & \verb|\newcite| \\
  \citeyearpar{Gusfield:97} & \verb|\citeyearpar| & \verb|\shortcite| \\
\end{tabular}
\caption{Citation commands supported by the style file.
  The citation style is based on the natbib package and
  supports all natbib citation commands.
  It also supports commands defined in previous ACL style files
  for compatibility.
  }
\end{table*}

{\bf Citations}: Citations within the text appear in parentheses
as~\cite{Gusfield:97} or, if the author's name appears in the text
itself, as Gusfield~\shortcite{Gusfield:97}.
Using the provided \LaTeX\ style, the former is accomplished using
{\small\verb|\cite|} and the latter with {\small\verb|\shortcite|} or {\small\verb|\newcite|}.  Collapse multiple citations as in~\cite{Gusfield:97,Aho:72}; this is accomplished with the provided style using commas within the {\small\verb|\cite|} command, {\em e.g.}, {\small\verb|\cite{Gusfield:97,Aho:72}|}.  
Append lowercase letters to the year in cases of ambiguities.  
 Treat double authors as
in~\cite{Aho:72}, but write as in~\cite{Chandra:81} when more than two
authors are involved. Collapse multiple citations as
in~\cite{Gusfield:97,Aho:72}. Also refrain from using full citations
as sentence constituents.

\penalty -5000

We suggest that instead of
\begin{quote}
  ``\cite{Gusfield:97} showed that ...''
\end{quote}
you use
\begin{quote}
``Gusfield \shortcite{Gusfield:97}   showed that ...''
\end{quote}

If you are using the provided \LaTeX{} and Bib\TeX{} style files, you
can use the command \verb|\citet| (cite in text)
to get ``author (year)'' citations.

If the Bib\TeX{} file contains DOI fields, the paper
title in the references section will appear as a hyperlink
to the DOI, using the hyperref \LaTeX{} package.
To disable the hyperref package, load the style file
with the \verb|nohyperref| option:
\verb|\usepackage[nohyperref]{acl2017}|

\textbf{Digital Object Identifiers}:  As part of our work to make ACL
materials more widely used and cited outside of our discipline, ACL
has registered as a CrossRef member, as a registrant of Digital Object
Identifiers (DOIs), the standard for registering permanent URNs for
referencing scholarly materials.  As of 2017, we are requiring all
camera-ready references to contain the appropriate DOIs (or as a
second resort, the hyperlinked ACL Anthology Identifier) to all cited
works.  Thus, please ensure that you use Bib\TeX records that contain
DOI or URLs for any of the ACL materials that you reference.
Appropriate records should be found for most materials in the current
ACL Anthology at \url{http://aclanthology.info/}.

As examples, we cite \cite{P16-1001} to show you how papers with a DOI
will appear in the bibliography.  We cite \cite{C14-1001} to show how
papers without a DOI but with an ACL Anthology Identifier will appear
in the bibliography.  

As reviewing will be double-blind, the submitted version of the papers
should not include the authors' names and affiliations. Furthermore,
self-references that reveal the author's identity, {\em e.g.},
\begin{quote}
``We previously showed \cite{Gusfield:97} ...''  
\end{quote}
should be avoided. Instead, use citations such as 
\begin{quote}
``\citeauthor{Gusfield:97} \shortcite{Gusfield:97}
previously showed ... ''
\end{quote}

\textbf{Please do not use anonymous citations} and do not include
acknowledgements when submitting your papers. Papers that do not
conform to these requirements may be rejected without review.

\textbf{References}: Gather the full set of references together under
the heading {\bf References}; place the section before any Appendices,
unless they contain references. Arrange the references alphabetically
by first author, rather than by order of occurrence in the text.
Provide as complete a citation as possible, using a consistent format,
such as the one for {\em Computational Linguistics\/} or the one in the 
{\em Publication Manual of the American 
Psychological Association\/}~\cite{APA:83}.  Use of full names for
authors rather than initials is preferred.  A list of abbreviations
for common computer science journals can be found in the ACM 
{\em Computing Reviews\/}~\cite{ACM:83}.

The \LaTeX{} and Bib\TeX{} style files provided roughly fit the
American Psychological Association format, allowing regular citations, 
short citations and multiple citations as described above.

{\bf Appendices}: Appendices, if any, directly follow the text and the
references (but see above).  Letter them in sequence and provide an
informative title: {\bf Appendix A. Title of Appendix}.

\subsection{Footnotes}

{\bf Footnotes}: Put footnotes at the bottom of the page and use 9
points text. They may be numbered or referred to by asterisks or other
symbols.\footnote{This is how a footnote should appear.} Footnotes
should be separated from the text by a line.\footnote{Note the line
separating the footnotes from the text.}

\subsection{Graphics}

{\bf Illustrations}: Place figures, tables, and photographs in the
paper near where they are first discussed, rather than at the end, if
possible.  Wide illustrations may run across both columns.  Color
illustrations are discouraged, unless you have verified that  
they will be understandable when printed in black ink.

{\bf Captions}: Provide a caption for every illustration; number each one
sequentially in the form:  ``Figure 1. Caption of the Figure.'' ``Table 1.
Caption of the Table.''  Type the captions of the figures and 
tables below the body, using 11 point text.

\subsection{Accessibility}
\label{ssec:accessibility}

In an effort to accommodate the color-blind (as well as those printing
to paper), grayscale readability for all accepted papers will be
encouraged.  Color is not forbidden, but authors should ensure that
tables and figures do not rely solely on color to convey critical
distinctions.
Here we give a simple criterion on your colored figures, if your paper has to be printed in black and white, then you must assure that every curves or points in your figures can be still clearly distinguished.

% Min: no longer used as of ACL 2017, following ACL exec's decision to
% remove this extra workflow that was not executed much.
% BEGIN: remove
%% \section{XML conversion and supported \LaTeX\ packages}

%% Following ACL 2014 we will also we will attempt to automatically convert 
%% your \LaTeX\ source files to publish papers in machine-readable 
%% XML with semantic markup in the ACL Anthology, in addition to the 
%% traditional PDF format.  This will allow us to create, over the next 
%% few years, a growing corpus of scientific text for our own future research, 
%% and picks up on recent initiatives on converting ACL papers from earlier 
%% years to XML. 

%% We encourage you to submit a ZIP file of your \LaTeX\ sources along
%% with the camera-ready version of your paper. We will then convert them
%% to XML automatically, using the LaTeXML tool
%% (\url{http://dlmf.nist.gov/LaTeXML}). LaTeXML has \emph{bindings} for
%% a number of \LaTeX\ packages, including the ACL 2017 stylefile. These
%% bindings allow LaTeXML to render the commands from these packages
%% correctly in XML. For best results, we encourage you to use the
%% packages that are officially supported by LaTeXML, listed at
%% \url{http://dlmf.nist.gov/LaTeXML/manual/included.bindings}
% END: remove

\section{Translation of non-English Terms}

It is also advised to supplement non-English characters and terms
with appropriate transliterations and/or translations
since not all readers understand all such characters and terms.
Inline transliteration or translation can be represented in
the order of: original-form transliteration ``translation''.

\section{Length of Submission}
\label{sec:length}

The ACL 2017 main conference accepts submissions of long papers and
short papers.
 Long papers may consist of up to eight (8) pages of
content plus unlimited pages for references. Upon acceptance, final
versions of long papers will be given one additional page -- up to nine (9)
pages of content plus unlimited pages for references -- so that reviewers' comments
can be taken into account. Short papers may consist of up to four (4)
pages of content, plus unlimited pages for references. Upon
acceptance, short papers will be given five (5) pages in the
proceedings and unlimited pages for references. 

For both long and short papers, all illustrations and tables that are part
of the main text must be accommodated within these page limits, observing
the formatting instructions given in the present document. Supplementary
material in the form of appendices does not count towards the page limit.

However, note that supplementary material should be supplementary
(rather than central) to the paper, and that reviewers may ignore
supplementary material when reviewing the paper (see Appendix
\ref{sec:supplemental}). Papers that do not conform to the specified
length and formatting requirements are subject to be rejected without
review.

Workshop chairs may have different rules for allowed length and
whether supplemental material is welcome. As always, the respective
call for papers is the authoritative source.

\section*{Acknowledgments}

The acknowledgments should go immediately before the references.  Do
not number the acknowledgments section. Do not include this section
when submitting your paper for review.

% include your own bib file like this:
%\bibliographystyle{acl}
%\bibliography{acl2017}
\bibliography{acl2017}
\bibliographystyle{acl_natbib}

\appendix

\section{Supplemental Material}
\label{sec:supplemental}
ACL 2017 also encourages the submission of supplementary material
to report preprocessing decisions, model parameters, and other details
necessary for the replication of the experiments reported in the 
paper. Seemingly small preprocessing decisions can sometimes make
a large difference in performance, so it is crucial to record such
decisions to precisely characterize state-of-the-art methods.

Nonetheless, supplementary material should be supplementary (rather
than central) to the paper. {\bf Submissions that misuse the supplementary 
material may be rejected without review.}
Essentially, supplementary material may include explanations or details
of proofs or derivations that do not fit into the paper, lists of
features or feature templates, sample inputs and outputs for a system,
pseudo-code or source code, and data. (Source code and data should
be separate uploads, rather than part of the paper).

The paper should not rely on the supplementary material: while the paper
may refer to and cite the supplementary material and the supplementary material will be available to the
reviewers, they will not be asked to review the
supplementary material.

Appendices ({\em i.e.} supplementary material in the form of proofs, tables,
or pseudo-code) should come after the references, as shown here. Use
\verb|\appendix| before any appendix section to switch the section
numbering over to letters.

\section{Multiple Appendices}
\dots can be gotten by using more than one section. We hope you won't
need that.
\fi

==> combating-human-trafficking-2 2/content/goodideas.tex <==
The way they write things is similar. The second intuition, we can handle misspelling by using context. One hot vector is large. 
Large enough vector we capture variations of that
The way they write everything else is as informative

Asian with $ removed and show that it is still performing good!

One for english dictionary, should be tried to be encoded with character level


NOT SO IMportant
-- Replacement studies. 2

-- precision vs recal curve 2 
--1 hot lstm

TODO:
-- Add Random to the table
-- TNSE on visual features
-- weighted accuracy 9
-- Agreements both in alpha and also for percentage.
-- Human performance 


-- Wordvector distance studies 9
-- Multimodal SVM?

==> combating-human-trafficking-2 2/figs/AdLength.tex <==
\begin{figure}[t!]
  \centering
  %\includegraphics[width=0.5\textwidth]{figs/adlen.pdf}
  \begin{tikzpicture}
    \begin{axis}
      [
        width=0.45\textwidth,
        height=2in,
        bar width=6.5pt,
        ybar stacked,
        legend pos=north west,
        title={Advertisement lengths},
        xlabel={Number of unigrams},
        xtick={0,40,...,200},
        extra x ticks={230},
        extra x tick labels={$+$},
      ]
      \addplot table[x=max, y=pos] {data/advertisement_lengths_bins.dat};
      \addplot table[x=max, y=neg] {data/advertisement_lengths_bins.dat};
      \addlegendentry{Positive}
      \addlegendentry{Negative}
    \end{axis}
  \end{tikzpicture}
  \caption{Distribution of the length of advertisements in Trafficking-10k. There is no significant difference between positive and negative cases purely based on length.}
  \label{fig:adlen}
\end{figure}

==> combating-human-trafficking-2 2/figs/CharacterFig.tex <==
\begin{figure}[t]
	\centering
	\includegraphics[width=0.5\textwidth]{lengthplot.png}
	\caption{Coverage of Advertisements Based on Advertisement Length. Both positive and negative classes show similar distribution. }
	\label{figure:lengthplot}
\end{figure}

==> combating-human-trafficking-2 2/figs/OverviewFig.tex <==
\begin{figure*}[t]
	\centering
	\includegraphics[width=0.9\textwidth]{figs/overview-2.pdf}
	\caption{Overview of our proposed Human Trafficking Deep Network (HTDN). The input to HTDN is text and a set of 5 images. The text goes through the Language Network $\mathcal{F}_l$ to get the language representation $h_l$ and the set of 5 images go through the Vision Network $\mathcal{F}_v$ to get the visual representation $h_v$. $h_l$ and $h_v$ are then fused together to get the multimodal representation $h_m$. The Convolutional Decision Network $\mathcal{F}_d$ conditioned on the $h_m$ makes inference about whether or not the advertisement is suspected of trafficking} 
	\label{fig:overview}
\end{figure*}

==> combating-human-trafficking-2 2/figs/TSNEFig.tex <==

\begin{figure*}[th!]
  \centering
  % Note: raster graphics used here, because the PDF ones are extremely complicated and slow renderers to a crawl.
  \includegraphics[width=0.5\textwidth]{figs/vis_data_exp_binary_raster}%
  \includegraphics[width=0.5\textwidth]{figs/vis_data_nonexp_binary_raster}%
  \\\medskip
  \includegraphics[width=0.5\textwidth]{figs/vis_data_wordv_avg_raster}%
  \includegraphics[width=0.5\textwidth]{figs/vis_data_img_raster}%
  \caption{%
    2D t-SNE representation of different input features for baseline models.
    Clockwise from top left: one hot vectors with expert data, one hot vectors without expert data, visual features from Vision Network $\mathcal{F}_v$, and average word vectors.
    These representations show that inference is not trivial in Trafficking-10k dataset.
  }
  \label{fig:tsne}
\end{figure*}

==> combating-human-trafficking-2 2/figs/USMapFig.tex <==
\begin{figure}[t!]
	\centering
	\includegraphics[width=0.5\textwidth]{figs/nasa.png}
	\caption{Distribution of advertisements in Trafficking-10k dataset across United States and Canada.}
	\label{fig:usmap}
\end{figure}

==> combating-human-trafficking-2 2/tables/AgreementTable.tex <==
% TODO: Fill in with actual values
\begin{table}[t]
	\centering
	\begin{tabular}{ c | c  c  c  c  c }
	 & MA1 & MA2 & MA3 & LEO1 & LEO2 \\
	%\hhline{|=#=====|}
    \hline
	MA1 & -- & 0.59 & 0.66 & 0.24 & 0.32 \\
	MA2 & 0.59 & -- & 0.69 & 0.30 & 0.46 \\
	MA3 & 0.66 & 0.69 & -- & 0.28 & 0.38 \\
	LEO1 & 0.24 & 0.30 & 0.28 & -- & 0.28 \\
	LEO2 & 0.32 & 0.46 & 0.38 & 0.28 & -- \\
	\end{tabular}
	\caption{Ordinal Krippendorff's Alpha Annotator Agreement Values}
    \label{tab:ordannotagreements}
\end{table}



% TODO: Fill in with actual values
\begin{table}[t]
	\centering
	\begin{tabular}{| c || c | c | c | c | c |}
	\hline
	-- & MA1 & MA2 & MA3 & LEO1 & LEO2 \\
	\hhline{|=#=|=|=|=|=|}
	MA1 & -- & 0.55 & 0.57 & 0.40 & 1 \\
	\hline
	MA2 & 0.55 & -- & 1 & 1 & 1 \\
	\hline
	MA3 & 0.57 & 1 & -- & 1 & 1 \\
	\hline
	LEO1 & 0.40 & 1 & 1 & -- & 1 \\
	\hline
	LEO2 & 1 & 1 & 1 & 1 & -- \\
	\hline
	\end{tabular}
	\caption{Binary Krippendorff's Alpha Annotator Agreement Values}
    \label{tab:binannotagreements}
\end{table}

==> combating-human-trafficking-2 2/tables/ResultsTable.tex <==
\begin{table*}[t!]
  \centering
  \newcommand{\category}[1]{\rlap{\textbf{#1}}}
  \newcommand{\entry}{\quad}
  \begin{tabular}{l*5r}
    \toprule
    \textbf{Model} & \textbf{Wt.\ Acc.\ (\%)} & \textbf{F1 (\%)} & \textbf{Acc.\ (\%)} & \textbf{Precision (\%)} & \textbf{Recall (\%)} \\
    \midrule
	\category{Random}                  & 50.0          & -          & 68.2 & - & -   \\
    %
    \category{Keywords} \\
    \entry Random Forest              & 67.0          & 55.2          & 78.1 & 78.2 & 42.6   \\
    \entry Logistic Regression        & 69.9          & 57.8          & 78.4 & 75.5 & 46.8   \\
    \entry Linear SVM                 & 69.5          & 57.0          & 78.6 & 78.0 & 44.9   \\[1ex]
    %
    \category{Average Trafficking Vectors} \\
    \entry Random Forest              & 67.3          & 54.1          & 78.0 & 79.3 & 41.1   \\
    \entry Logistic Regression        & 72.2          & 61.7          & 80.2 & 79.2 & 50.6   \\
    \entry Linear SVM                 & 70.3          & 57.7          & 79.2 & 80.7 & 44.9   \\[1ex]
    %
    \category{108 One-Hot} \\
    \entry Random Forest              & 62.4          & 60.7          & 72.6 & 61.5 & 60.0   \\
    \entry Logistic Regression        & 62.5          & 45.1          & 72.2 & 60.0 & 36.1   \\
    \entry Linear SVM                 & 61.7          & 45.1          & 71.8 & 58.6 & 36.7   \\[1ex]
    %
    \category{Bag of Words} \\
    \entry Random Forest              & 57.6          & 24.5          & 70.4 & 63.2 & 15.2   \\
    \entry Logistic Regression        & 71.1          & 24.5          & 70.4 & 63.2 & 15.2   \\
    \entry Linear SVM                 & 71.2          & 24.5          & 70.4 & 63.2 & 15.2   \\[1ex]
    %
    \category{HTDN Unimodal} \\
    \entry $\mathcal{F}_{l}$          & 74.5          & 65.8          & 78.8 & 69.8 & 62.3   \\
    \entry $\mathcal{F}_{v}$ [VGG]    & 69.1          & 58.4          & 74.2 & 66.7 & 52.0   \\
    \entry $\mathcal{F}_{v}$ [T-VGG]  & 70.4          & {59.5}        & 77.3 & 78.3 & 48.0   \\[1ex]
    %
    \category{HTDN}                   & \textbf{75.3} & \textbf{66.5} & 80.0 & 71.4 & 62.2   \\[1ex]
    %
    \category{Human}                  & 83.7          & 73.7          & 84.0 & 76.7 & 70.9   \\
    %
    \bottomrule
  \end{tabular}
  \caption{Results of our experiments. We compare our HTDN model to various baselines using different inputs. HTDN ourperforms other baselines in both weighted accuracy and F-score.}
  \label{table:results}
\end{table*}

==> content/done.tex <==
-- Statistics for the ads, how many unigrams (106954), images (60337), bigrams (353324), trigrams (565403), characters including spaces and punctuation and hex, excluding newline (182), average length of ad (avg 137 words, stddev 74, median 133, min 7, max 1810), average number of images (avg 5.9, median 5, mode 4, stddev 4.6, min 0, max 90), average length of trafficking ads (avg 134 words, stddev 39, median 136, min 12, max 666) , average length of non-trafficking ads (avg 141, stddev 85, median 131, min 7, max 1810), number of trafficking ads (3257), number of non-trafficking ads (6992), couple of other ideas for visualizing the trafficking stuff, such as look at MOSI sentiment paper figure 2. 9

-- How many n-grams are out if we use glove 9
-- Recalculate f1. 
-- Overview figure -- william

==> content/dummy.tex <==
\iffalse
\begin{figure*}
\centering
\begin{tikzpicture}
\begin{axis}[
xlabel style={font={\small}},
xlabel={Hey!},
legend pos={outer north east},
width=5in,
title=Hello,
]
\addplot table {fscorevsubprob.dat};
\addlegendentry{RF-F}
\addplot table[y index={2}] {fscorevsubprob.dat};
\addlegendentry{SVM-F}
\addplot table[y index={3}] {fscorevsubprob.dat};
\addlegendentry{LR-F}
\addplot table[y index={4}] {fscorevsubprob.dat};
\addlegendentry{cLSTM-F}
\end{axis}
\end{tikzpicture}
\end{figure*}
\fi
\iffalse
\section{Credits}

This document has been adapted from the instructions for earlier ACL
and NAACL proceedings, including those for ACL 2017 by Dan Gildea and
Min-Yen Kan, NAACL-2017 by Margaret Mitchell, ACL-2012 by Maggie Li
and Michael White, those from ACL-2010 by Jing-Shing Chang and Philipp
Koehn, those for ACL-2008 by Johanna D. Moore, Simone Teufel, James
Allan, and Sadaoki Furui, those for ACL-2005 by Hwee Tou Ng and Kemal
Oflazer, those for ACL-2002 by Eugene Charniak and Dekang Lin, and
earlier ACL and EACL formats. Those versions were written by several
people, including John Chen, Henry S. Thompson and Donald
Walker. Additional elements were taken from the formatting
instructions of the {\em International Joint Conference on Artificial
  Intelligence} and the \emph{Conference on Computer Vision and
  Pattern Recognition}.

\section{Introduction}

The following instructions are directed to authors of papers submitted
to ACL-2017 or accepted for publication in its proceedings. All
authors are required to adhere to these specifications. Authors are
required to provide a Portable Document Format (PDF) version of their
papers. \textbf{The proceedings are designed for printing on A4
paper.}

\section{General Instructions}

Manuscripts must be in two-column format.  Exceptions to the
two-column format include the title, authors' names and complete
addresses, which must be centered at the top of the first page, and
any full-width figures or tables (see the guidelines in
Subsection~\ref{ssec:first}). {\bf Type single-spaced.}  Start all
pages directly under the top margin. See the guidelines later
regarding formatting the first page.  The manuscript should be
printed single-sided and its length
should not exceed the maximum page limit described in Section~\ref{sec:length}.
Pages are numbered for  initial submission. However, {\bf do not number the pages in the camera-ready version}.

By uncommenting {\small\verb|\aclfinalcopy|} at the top of this 
 document, it will compile to produce an example of the camera-ready formatting; by leaving it commented out, the document will be anonymized for initial submission.  When you first create your submission on softconf, please fill in your submitted paper ID where {\small\verb|***|} appears in the {\small\verb|\def\aclpaperid{***}|} definition at the top.

The review process is double-blind, so do not include any author information (names, addresses) when submitting a paper for review.  
However, you should maintain space for names and addresses so that they will fit in the final (accepted) version.  The ACL 2017 \LaTeX\ style will create a titlebox space of 2.5in for you when {\small\verb|\aclfinalcopy|} is commented out.  

\subsection{The Ruler}
The ACL 2017 style defines a printed ruler which should be presented in the
version submitted for review.  The ruler is provided in order that
reviewers may comment on particular lines in the paper without
circumlocution.  If you are preparing a document without the provided
style files, please arrange for an equivalent ruler to
appear on the final output pages.  The presence or absence of the ruler
should not change the appearance of any other content on the page.  The
camera ready copy should not contain a ruler. (\LaTeX\ users may uncomment
the {\small\verb|\aclfinalcopy|} command in the document preamble.)  

Reviewers: note that the ruler measurements do not align well with
lines in the paper -- this turns out to be very difficult to do well
when the paper contains many figures and equations, and, when done,
looks ugly. In most cases one would expect that the approximate
location will be adequate, although you can also use fractional
references ({\em e.g.}, the first paragraph on this page ends at mark $114.5$).

\subsection{Electronically-available resources}

ACL provides this description in \LaTeX2e{} ({\small\tt acl2017.tex}) and PDF
format ({\small\tt acl2017.pdf}), along with the \LaTeX2e{} style file used to
format it ({\small\tt acl2017.sty}) and an ACL bibliography style ({\small\tt acl\_natbib.bst})
and example bibliography ({\small\tt acl2017.bib}).
These files are all available at
{\small\tt acl2017.org/index.php?article\_id=9}. We
strongly recommend the use of these style files, which have been
appropriately tailored for the ACL 2017 proceedings.

\subsection{Format of Electronic Manuscript}
\label{sect:pdf}

For the production of the electronic manuscript you must use Adobe's
Portable Document Format (PDF). PDF files are usually produced from
\LaTeX\ using the \textit{pdflatex} command. If your version of
\LaTeX\ produces Postscript files, you can convert these into PDF
using \textit{ps2pdf} or \textit{dvipdf}. On Windows, you can also use
Adobe Distiller to generate PDF.

Please make sure that your PDF file includes all the necessary fonts
(especially tree diagrams, symbols, and fonts with Asian
characters). When you print or create the PDF file, there is usually
an option in your printer setup to include none, all or just
non-standard fonts.  Please make sure that you select the option of
including ALL the fonts. \textbf{Before sending it, test your PDF by
  printing it from a computer different from the one where it was
  created.} Moreover, some word processors may generate very large PDF
files, where each page is rendered as an image. Such images may
reproduce poorly. In this case, try alternative ways to obtain the
PDF. One way on some systems is to install a driver for a postscript
printer, send your document to the printer specifying ``Output to a
file'', then convert the file to PDF.

It is of utmost importance to specify the \textbf{A4 format} (21 cm
x 29.7 cm) when formatting the paper. When working with
{\tt dvips}, for instance, one should specify {\tt -t a4}.
Or using the command \verb|\special{papersize=210mm,297mm}| in the latex
preamble (directly below the \verb|\usepackage| commands). Then using 
{\tt dvipdf} and/or {\tt pdflatex} which would make it easier for some.

Print-outs of the PDF file on A4 paper should be identical to the
hardcopy version. If you cannot meet the above requirements about the
production of your electronic submission, please contact the
publication chairs as soon as possible.

\subsection{Layout}
\label{ssec:layout}

Format manuscripts two columns to a page, in the manner these
instructions are formatted. The exact dimensions for a page on A4
paper are:

\begin{itemize}
\item Left and right margins: 2.5 cm
\item Top margin: 2.5 cm
\item Bottom margin: 2.5 cm
\item Column width: 7.7 cm
\item Column height: 24.7 cm
\item Gap between columns: 0.6 cm
\end{itemize}

\noindent Papers should not be submitted on any other paper size.
 If you cannot meet the above requirements about the production of 
 your electronic submission, please contact the publication chairs 
 above as soon as possible.

\subsection{Fonts}

For reasons of uniformity, Adobe's {\bf Times Roman} font should be
used. In \LaTeX2e{} this is accomplished by putting

\begin{quote}
\begin{verbatim}
\usepackage{times}
\usepackage{latexsym}
\end{verbatim}
\end{quote}
in the preamble. If Times Roman is unavailable, use {\bf Computer
  Modern Roman} (\LaTeX2e{}'s default).  Note that the latter is about
  10\% less dense than Adobe's Times Roman font.

\begin{table}[h]
\begin{center}
\begin{tabular}{|l|rl|}
\hline \bf Type of Text & \bf Font Size & \bf Style \\ \hline
paper title & 15 pt & bold \\
author names & 12 pt & bold \\
author affiliation & 12 pt & \\
the word ``Abstract'' & 12 pt & bold \\
section titles & 12 pt & bold \\
document text & 11 pt  &\\
captions & 11 pt & \\
abstract text & 10 pt & \\
bibliography & 10 pt & \\
footnotes & 9 pt & \\
\hline
\end{tabular}
\end{center}
\caption{\label{font-table} Font guide. }
\end{table}

\subsection{The First Page}
\label{ssec:first}

Center the title, author's name(s) and affiliation(s) across both
columns. Do not use footnotes for affiliations. Do not include the
paper ID number assigned during the submission process. Use the
two-column format only when you begin the abstract.

{\bf Title}: Place the title centered at the top of the first page, in
a 15-point bold font. (For a complete guide to font sizes and styles,
see Table~\ref{font-table}) Long titles should be typed on two lines
without a blank line intervening. Approximately, put the title at 2.5
cm from the top of the page, followed by a blank line, then the
author's names(s), and the affiliation on the following line. Do not
use only initials for given names (middle initials are allowed). Do
not format surnames in all capitals ({\em e.g.}, use ``Mitchell'' not
``MITCHELL'').  Do not format title and section headings in all
capitals as well except for proper names (such as ``BLEU'') that are
conventionally in all capitals.  The affiliation should contain the
author's complete address, and if possible, an electronic mail
address. Start the body of the first page 7.5 cm from the top of the
page.

The title, author names and addresses should be completely identical
to those entered to the electronical paper submission website in order
to maintain the consistency of author information among all
publications of the conference. If they are different, the publication
chairs may resolve the difference without consulting with you; so it
is in your own interest to double-check that the information is
consistent.

{\bf Abstract}: Type the abstract at the beginning of the first
column. The width of the abstract text should be smaller than the
width of the columns for the text in the body of the paper by about
0.6 cm on each side. Center the word {\bf Abstract} in a 12 point bold
font above the body of the abstract. The abstract should be a concise
summary of the general thesis and conclusions of the paper. It should
be no longer than 200 words. The abstract text should be in 10 point font.

{\bf Text}: Begin typing the main body of the text immediately after
the abstract, observing the two-column format as shown in 
the present document. Do not include page numbers.

{\bf Indent}: When starting a new paragraph. Use 11 points for text and 
subsection headings, 12 points for section headings and 15 points for
the title. 

\begin{table}
\centering
\small
\begin{tabular}{cc}
\begin{tabular}{|l|l|}
\hline
{\bf Command} & {\bf Output}\\\hline
\verb|{\"a}| & {\"a} \\
\verb|{\^e}| & {\^e} \\
\verb|{\`i}| & {\`i} \\ 
\verb|{\.I}| & {\.I} \\ 
\verb|{\o}| & {\o} \\
\verb|{\'u}| & {\'u}  \\ 
\verb|{\aa}| & {\aa}  \\\hline
\end{tabular} & 
\begin{tabular}{|l|l|}
\hline
{\bf Command} & {\bf  Output}\\\hline
\verb|{\c c}| & {\c c} \\ 
\verb|{\u g}| & {\u g} \\ 
\verb|{\l}| & {\l} \\ 
\verb|{\~n}| & {\~n} \\ 
\verb|{\H o}| & {\H o} \\ 
\verb|{\v r}| & {\v r} \\ 
\verb|{\ss}| & {\ss} \\\hline
\end{tabular}
\end{tabular}
\caption{Example commands for accented characters, to be used in, {\em e.g.}, \BibTeX\ names.}\label{tab:accents}
\end{table}

\subsection{Sections}

{\bf Headings}: Type and label section and subsection headings in the
style shown on the present document.  Use numbered sections (Arabic
numerals) in order to facilitate cross references. Number subsections
with the section number and the subsection number separated by a dot,
in Arabic numerals. Do not number subsubsections.

\begin{table*}
\centering
\begin{tabular}{lll}
  output & natbib & previous ACL style files\\
  \hline
  \citep{Gusfield:97} & \verb|\citep| & \verb|\cite| \\
  \citet{Gusfield:97} & \verb|\citet| & \verb|\newcite| \\
  \citeyearpar{Gusfield:97} & \verb|\citeyearpar| & \verb|\shortcite| \\
\end{tabular}
\caption{Citation commands supported by the style file.
  The citation style is based on the natbib package and
  supports all natbib citation commands.
  It also supports commands defined in previous ACL style files
  for compatibility.
  }
\end{table*}

{\bf Citations}: Citations within the text appear in parentheses
as~\cite{Gusfield:97} or, if the author's name appears in the text
itself, as Gusfield~\shortcite{Gusfield:97}.
Using the provided \LaTeX\ style, the former is accomplished using
{\small\verb|\cite|} and the latter with {\small\verb|\shortcite|} or {\small\verb|\newcite|}.  Collapse multiple citations as in~\cite{Gusfield:97,Aho:72}; this is accomplished with the provided style using commas within the {\small\verb|\cite|} command, {\em e.g.}, {\small\verb|\cite{Gusfield:97,Aho:72}|}.  
Append lowercase letters to the year in cases of ambiguities.  
 Treat double authors as
in~\cite{Aho:72}, but write as in~\cite{Chandra:81} when more than two
authors are involved. Collapse multiple citations as
in~\cite{Gusfield:97,Aho:72}. Also refrain from using full citations
as sentence constituents.

\penalty -5000

We suggest that instead of
\begin{quote}
  ``\cite{Gusfield:97} showed that ...''
\end{quote}
you use
\begin{quote}
``Gusfield \shortcite{Gusfield:97}   showed that ...''
\end{quote}

If you are using the provided \LaTeX{} and Bib\TeX{} style files, you
can use the command \verb|\citet| (cite in text)
to get ``author (year)'' citations.

If the Bib\TeX{} file contains DOI fields, the paper
title in the references section will appear as a hyperlink
to the DOI, using the hyperref \LaTeX{} package.
To disable the hyperref package, load the style file
with the \verb|nohyperref| option:
\verb|\usepackage[nohyperref]{acl2017}|

\textbf{Digital Object Identifiers}:  As part of our work to make ACL
materials more widely used and cited outside of our discipline, ACL
has registered as a CrossRef member, as a registrant of Digital Object
Identifiers (DOIs), the standard for registering permanent URNs for
referencing scholarly materials.  As of 2017, we are requiring all
camera-ready references to contain the appropriate DOIs (or as a
second resort, the hyperlinked ACL Anthology Identifier) to all cited
works.  Thus, please ensure that you use Bib\TeX records that contain
DOI or URLs for any of the ACL materials that you reference.
Appropriate records should be found for most materials in the current
ACL Anthology at \url{http://aclanthology.info/}.

As examples, we cite \cite{P16-1001} to show you how papers with a DOI
will appear in the bibliography.  We cite \cite{C14-1001} to show how
papers without a DOI but with an ACL Anthology Identifier will appear
in the bibliography.  

As reviewing will be double-blind, the submitted version of the papers
should not include the authors' names and affiliations. Furthermore,
self-references that reveal the author's identity, {\em e.g.},
\begin{quote}
``We previously showed \cite{Gusfield:97} ...''  
\end{quote}
should be avoided. Instead, use citations such as 
\begin{quote}
``\citeauthor{Gusfield:97} \shortcite{Gusfield:97}
previously showed ... ''
\end{quote}

\textbf{Please do not use anonymous citations} and do not include
acknowledgements when submitting your papers. Papers that do not
conform to these requirements may be rejected without review.

\textbf{References}: Gather the full set of references together under
the heading {\bf References}; place the section before any Appendices,
unless they contain references. Arrange the references alphabetically
by first author, rather than by order of occurrence in the text.
Provide as complete a citation as possible, using a consistent format,
such as the one for {\em Computational Linguistics\/} or the one in the 
{\em Publication Manual of the American 
Psychological Association\/}~\cite{APA:83}.  Use of full names for
authors rather than initials is preferred.  A list of abbreviations
for common computer science journals can be found in the ACM 
{\em Computing Reviews\/}~\cite{ACM:83}.

The \LaTeX{} and Bib\TeX{} style files provided roughly fit the
American Psychological Association format, allowing regular citations, 
short citations and multiple citations as described above.

{\bf Appendices}: Appendices, if any, directly follow the text and the
references (but see above).  Letter them in sequence and provide an
informative title: {\bf Appendix A. Title of Appendix}.

\subsection{Footnotes}

{\bf Footnotes}: Put footnotes at the bottom of the page and use 9
points text. They may be numbered or referred to by asterisks or other
symbols.\footnote{This is how a footnote should appear.} Footnotes
should be separated from the text by a line.\footnote{Note the line
separating the footnotes from the text.}

\subsection{Graphics}

{\bf Illustrations}: Place figures, tables, and photographs in the
paper near where they are first discussed, rather than at the end, if
possible.  Wide illustrations may run across both columns.  Color
illustrations are discouraged, unless you have verified that  
they will be understandable when printed in black ink.

{\bf Captions}: Provide a caption for every illustration; number each one
sequentially in the form:  ``Figure 1. Caption of the Figure.'' ``Table 1.
Caption of the Table.''  Type the captions of the figures and 
tables below the body, using 11 point text.

\subsection{Accessibility}
\label{ssec:accessibility}

In an effort to accommodate the color-blind (as well as those printing
to paper), grayscale readability for all accepted papers will be
encouraged.  Color is not forbidden, but authors should ensure that
tables and figures do not rely solely on color to convey critical
distinctions.
Here we give a simple criterion on your colored figures, if your paper has to be printed in black and white, then you must assure that every curves or points in your figures can be still clearly distinguished.

% Min: no longer used as of ACL 2017, following ACL exec's decision to
% remove this extra workflow that was not executed much.
% BEGIN: remove
%% \section{XML conversion and supported \LaTeX\ packages}

%% Following ACL 2014 we will also we will attempt to automatically convert 
%% your \LaTeX\ source files to publish papers in machine-readable 
%% XML with semantic markup in the ACL Anthology, in addition to the 
%% traditional PDF format.  This will allow us to create, over the next 
%% few years, a growing corpus of scientific text for our own future research, 
%% and picks up on recent initiatives on converting ACL papers from earlier 
%% years to XML. 

%% We encourage you to submit a ZIP file of your \LaTeX\ sources along
%% with the camera-ready version of your paper. We will then convert them
%% to XML automatically, using the LaTeXML tool
%% (\url{http://dlmf.nist.gov/LaTeXML}). LaTeXML has \emph{bindings} for
%% a number of \LaTeX\ packages, including the ACL 2017 stylefile. These
%% bindings allow LaTeXML to render the commands from these packages
%% correctly in XML. For best results, we encourage you to use the
%% packages that are officially supported by LaTeXML, listed at
%% \url{http://dlmf.nist.gov/LaTeXML/manual/included.bindings}
% END: remove

\section{Translation of non-English Terms}

It is also advised to supplement non-English characters and terms
with appropriate transliterations and/or translations
since not all readers understand all such characters and terms.
Inline transliteration or translation can be represented in
the order of: original-form transliteration ``translation''.

\section{Length of Submission}
\label{sec:length}

The ACL 2017 main conference accepts submissions of long papers and
short papers.
 Long papers may consist of up to eight (8) pages of
content plus unlimited pages for references. Upon acceptance, final
versions of long papers will be given one additional page -- up to nine (9)
pages of content plus unlimited pages for references -- so that reviewers' comments
can be taken into account. Short papers may consist of up to four (4)
pages of content, plus unlimited pages for references. Upon
acceptance, short papers will be given five (5) pages in the
proceedings and unlimited pages for references. 

For both long and short papers, all illustrations and tables that are part
of the main text must be accommodated within these page limits, observing
the formatting instructions given in the present document. Supplementary
material in the form of appendices does not count towards the page limit.

However, note that supplementary material should be supplementary
(rather than central) to the paper, and that reviewers may ignore
supplementary material when reviewing the paper (see Appendix
\ref{sec:supplemental}). Papers that do not conform to the specified
length and formatting requirements are subject to be rejected without
review.

Workshop chairs may have different rules for allowed length and
whether supplemental material is welcome. As always, the respective
call for papers is the authoritative source.

\section*{Acknowledgments}

The acknowledgments should go immediately before the references.  Do
not number the acknowledgments section. Do not include this section
when submitting your paper for review.

% include your own bib file like this:
%\bibliographystyle{acl}
%\bibliography{acl2017}
\bibliography{acl2017}
\bibliographystyle{acl_natbib}

\appendix

\section{Supplemental Material}
\label{sec:supplemental}
ACL 2017 also encourages the submission of supplementary material
to report preprocessing decisions, model parameters, and other details
necessary for the replication of the experiments reported in the 
paper. Seemingly small preprocessing decisions can sometimes make
a large difference in performance, so it is crucial to record such
decisions to precisely characterize state-of-the-art methods.

Nonetheless, supplementary material should be supplementary (rather
than central) to the paper. {\bf Submissions that misuse the supplementary 
material may be rejected without review.}
Essentially, supplementary material may include explanations or details
of proofs or derivations that do not fit into the paper, lists of
features or feature templates, sample inputs and outputs for a system,
pseudo-code or source code, and data. (Source code and data should
be separate uploads, rather than part of the paper).

The paper should not rely on the supplementary material: while the paper
may refer to and cite the supplementary material and the supplementary material will be available to the
reviewers, they will not be asked to review the
supplementary material.

Appendices ({\em i.e.} supplementary material in the form of proofs, tables,
or pseudo-code) should come after the references, as shown here. Use
\verb|\appendix| before any appendix section to switch the section
numbering over to letters.

\section{Multiple Appendices}
\dots can be gotten by using more than one section. We hope you won't
need that.
\fi

==> content/goodideas.tex <==
The way they write things is similar. The second intuition, we can handle misspelling by using context. One hot vector is large. 
Large enough vector we capture variations of that
The way they write everything else is as informative

Asian with $ removed and show that it is still performing good!

One for english dictionary, should be tried to be encoded with character level


NOT SO IMportant
-- Replacement studies. 2

-- precision vs recal curve 2 
--1 hot lstm

TODO:
-- Add Random to the table
-- TNSE on visual features
-- weighted accuracy 9
-- Agreements both in alpha and also for percentage.
-- Human performance 


-- Wordvector distance studies 9
-- Multimodal SVM?

==> figs/CharacterFig.tex <==
\begin{figure}[t]
	\centering
	\includegraphics[width=0.5\textwidth]{lengthplot.png}
	\caption{Coverage of Advertisements Based on Advertisement Length. Both positive and negative classes show similar distribution. }
	\label{figure:lengthplot}
\end{figure}

==> tables/AgreementTable.tex <==
% TODO: Fill in with actual values
\begin{table}[t]
	\centering
	\begin{tabular}{ c | c  c  c  c  c }
	 & MA1 & MA2 & MA3 & LEO1 & LEO2 \\
	%\hhline{|=#=====|}
    \hline
	MA1 & -- & 0.59 & 0.66 & 0.24 & 0.32 \\
	MA2 & 0.59 & -- & 0.69 & 0.30 & 0.46 \\
	MA3 & 0.66 & 0.69 & -- & 0.28 & 0.38 \\
	LEO1 & 0.24 & 0.30 & 0.28 & -- & 0.28 \\
	LEO2 & 0.32 & 0.46 & 0.38 & 0.28 & -- \\
	\end{tabular}
	\caption{Ordinal Krippendorff's Alpha Annotator Agreement Values}
    \label{tab:ordannotagreements}
\end{table}



% TODO: Fill in with actual values
\begin{table}[t]
	\centering
	\begin{tabular}{| c || c | c | c | c | c |}
	\hline
	-- & MA1 & MA2 & MA3 & LEO1 & LEO2 \\
	\hhline{|=#=|=|=|=|=|}
	MA1 & -- & 0.55 & 0.57 & 0.40 & 1 \\
	\hline
	MA2 & 0.55 & -- & 1 & 1 & 1 \\
	\hline
	MA3 & 0.57 & 1 & -- & 1 & 1 \\
	\hline
	LEO1 & 0.40 & 1 & 1 & -- & 1 \\
	\hline
	LEO2 & 1 & 1 & 1 & 1 & -- \\
	\hline
	\end{tabular}
	\caption{Binary Krippendorff's Alpha Annotator Agreement Values}
    \label{tab:binannotagreements}
\end{table}
